Discrete Weierstrass-type representations

Discrete Weierstrass-type representations yield a construction method in discrete differential geometry for certain classes of discrete surfaces. We show that the known discrete Weierstrass-type representations of certain surface classes can be viewed as applications of the $\Omega$-dual transform to lightlike Gauss maps in Laguerre geometry. From this construction, further Weierstrass-type representations arise. As an application of the techniques we develop, we show that all discrete linear Weingarten surfaces of Bryant or Bianchi type locally arise via Weierstrass-type representations from discrete holomorhpic maps.

==> DiscreteOmegaSurfacesInR31.tex <==
In Laguerre geometry a \emph{discrete isothermic sphere congruence} is a net $x:\Z^2 \to \R^{3,1}$ that possesses a \emph{Christoffel dual net} $x^\ast:\Z^2 \to \R^{3,1}$, which is characterised by 
\begin{itemize}
	\item $x$ and $x^\ast$ are circular nets with parallel edges, and
	\item $A(x,x^\ast) =0$. 
\end{itemize}
Clearly, this relation is symmetric in $x$ and $x^\ast$, hence, $x^\ast$ is itself a discrete isothermic sphere congruence. 

Analogous to Demoulin's definition of $\Omega$-surfaces (see \cite{demoulin1911}, \cite{demoulin1911a}), we give the following

\begin{defi}\label{def:OmegaNet}
	A \emph{discrete $\Omega$-net} is an envelope $L = x + G$ of a discrete isothermic sphere congruence.
\end{defi}

\begin{defi}\label{def:OmegaTrafo}
	We say that two $\Omega$-nets $L, L^\ast$ are \emph{$\Omega$-dual nets} if there are Christoffel dual nets $x\in \Gamma L$ and $x^\ast \in \Gamma L^\ast$ and the lightlike Gau{ss} maps coincide, i.e., $G^\ast = G$.  
\end{defi}

\begin{bem}
	If $L=x+G$ is an $\Omega$ net, then we may take a Christoffel dual $x^\ast$ of $x$ and define $L^\ast = x^\ast + G$. $L^\ast$ is automatically an envelope of $x^\ast$ and, thus, an $\Omega$-dual net of $L$. 
\end{bem}

